Learning to Estimate Hidden Motions with Global Motion Aggregation

Occlusions pose a significant challenge to optical flow algorithms that rely on local evidences. We consider an occluded point to be one that is imaged in the first frame but not in the next, a slight overloading of the standard definition since it also includes points that move out-of-frame. Estimating the motion of these points is extremely difficult, particularly in the two-frame setting. Previous work relies on CNNs to learn occlusions, without much success, or requires multiple frames to reason about occlusions using temporal smoothness. In this paper, we argue that the occlusion problem can be better solved in the two-frame case by modelling image self-similarities. We introduce a global motion aggregation module, a transformer-based approach to find long-range dependencies between pixels in the first image, and perform global aggregation on the corresponding motion features. We demonstrate that the optical flow estimates in the occluded regions can be significantly improved without damaging the performance in non-occluded regions. This approach obtains new state-of-the-art results on the challenging Sintel dataset, improving the average end-point error by 13.6% on Sintel Final and 13.7% on Sintel Clean. At the time of submission, our method ranks first on these benchmarks among all published and unpublished approaches. Code is available at https://github.com/zacjiang/GMA

==> fig_arch.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/architecture.pdf}
        \caption{\textbf{Overall architecture.} Our proposed GMA module is highlighted
        in the shadowed area. The global motion feature is then concatenated with the local motion 
        features and context features. }
    \label{fig:overall}
    \end{subfigure}

    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{figures/gma.pdf}
        \caption{\textbf{Details of GMA.} To model the self-similarity 
        of the first frame, we first
        project the context feature map to a query feature map and a key feature map. We then
        apply dot product of the two feature maps and softmax to obtain an attention matrix, which 
        encodes feature space self-similarity. Similar to transformers, we also take the 
        dot product between the query feature map and a set of positional embedding vectors 
        which augments the attention matrix with positional information.         
        The motion features encoded from the correlation volume is first projected with value
        projector, then aggregated with the attention matrix, outputting the aggregated motion 
        features.}
    \label{fig:details}
    \end{subfigure}

    \caption{\textbf{Network architecture.} Our network is based on the existing work RAFT
    \cite{raft}. We demonstrate how our proposed GMA module is fitted in the existing framework
    in Figure~\ref{fig:overall} and we give the details of the GMA module in 
    Figure~\ref{fig:details}. The details of RAFT are omitted and the readers are encouraged to
    refer to the original paper.}
    \label{fig:architecture}
\end{figure*}

==> fig_qualitative.tex <==
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Frame 1}
         \includegraphics[width=\textwidth]{qualitative_1_figs/img_1_e.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Frame 2}
         \includegraphics[width=\textwidth]{qualitative_1_figs/img_2.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Flow (RAFT \cite{raft})}
         \includegraphics[width=\textwidth]{qualitative_1_figs/RAFT_flow_e.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Flow (ours)}
         \includegraphics[width=\textwidth]{qualitative_1_figs/ours_flow_e.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Flow (ground truth)}
         \includegraphics[width=\textwidth]{qualitative_1_figs/gt_flow.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Error (RAFT \cite{raft})}
         \includegraphics[width=\textwidth]{qualitative_1_figs/RAFT_error_e.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \caption*{Error (ours)}
         \includegraphics[width=\textwidth]{qualitative_1_figs/ours_error_e.png}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/img_1_e.png}
         \label{fig:input1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/img_2.png}
         \label{fig:input2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/RAFT_flow_e.png}
         \label{fig:raft}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/ours_flow_e.png}
         \label{fig:ours}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/gt_flow.png}
         \label{fig:ours}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/RAFT_error_e.png}
         \label{fig:ours}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.138\textwidth}
         \centering
         \includegraphics[width=\textwidth]{qualitative_2_figs/ours_error_e.png}
         \label{fig:ours}
     \end{subfigure}

     \caption{
     \textbf{Recovering hidden motions.}
     In row 1, the bottom left corner of the ground moves out-of-frame, but reasoning that it
     belongs to the background allows the motion to be recovered from other parts of the image. 
     In row 2, the girl's staff is mostly occluded in the second frame, but strong cues from the 
     visible parts can resolve its motion.
     Our approach can estimate many hidden motions despite the presence of occlusions.
     The flow maps and the error maps have been fetched from the Sintel server \cite{sintel}. 
     Best viewed on screen. 
     }
    \label{fig:qualitative}
\end{figure*}
